Ethical Aspects of ChatGPT in Software Engineering Research

ChatGPT can improve Software Engineering (SE) research practices by offering efficient, accessible information analysis and synthesis based on natural language interactions. However, ChatGPT could bring ethical challenges, encompassing plagiarism, privacy, data security, and the risk of generating biased or potentially detrimental data. This research aims to fill the given gap by elaborating on the key elements: motivators, demotivators, and ethical principles of using ChatGPT in SE research. To achieve this objective, we conducted a literature survey, identified the mentioned elements, and presented their relationships by developing a taxonomy. Further, the identified literature-based elements (motivators, demotivators, and ethical principles) were empirically evaluated by conducting a comprehensive questionnaire-based survey involving SE researchers. Additionally, we employed Interpretive Structure Modeling (ISM) approach to analyze the relationships between the ethical principles of using ChatGPT in SE research and develop a level based decision model. We further conducted a Cross-Impact Matrix Multiplication Applied to Classification (MICMAC) analysis to create a cluster-based decision model. These models aim to help SE researchers devise effective strategies for ethically integrating ChatGPT into SE research by following the identified principles through adopting the motivators and addressing the demotivators. The findings of this study will establish a benchmark for incorporating ChatGPT services in SE research with an emphasis on ethical considerations.

==> next.tex <==
\section{What next}
\label{sec:next}

The ultimate aim of this research project is the development of comprehensive guidelines for using ChatGPT in software engineering research. This study presents a taxonomy (Figure \ref{Fig.Mapping of motivators and demotivators against research ethics}), developed based on the preliminarily investigated motivators, demotivators, and their possible impact on ChatGPT ethics aspects. The next steps are conducting a comprehensive multivocal literature review and questionnaire survey study to refine and identify the additional motivators and demotivators across ethical aspects of using ChatGPT in software engineering research.  Below are the steps we will follow for the development of guidelines: 1) Perform an extensive multivocal literature review to identify a broader range of motivators, demotivators and their potential impact on ethical aspects. 2) Design a survey questionnaire targeting software engineering researchers to validate the findings of multivocal literature review and explore additional motivators, demotivators and ethical aspects of using ChatGpt in software engineering research.
3) Comparatively analyse the the findings of multivocal literature review and questionnaire survey. Identify common themes, trends, and patterns emerging from these data sources to create a taxonomy of motivators, demotivators and their relationship to the ethical aspects. 4) Draft a set of guidelines
 based on the revised taxonomy addressing the ethical concerns of using ChatGPT in software engineering research. The guidelines should consider the motivators, demotivators, and their possible impact on ethical principles. 5) Invite AI ethics, software engineering, and ChatGPT application experts to review the draft guidelines. Collect their feedback and insights to refine and validate the guidelines. Incorporate their feedback to ensure the guidelines are robust, relevant, and effective in addressing ethical concerns. 6) Conduct academic case studies to evaluate the set of guidelines in real-world software engineering research and incorporate the potential changes based on the case studies' findings.
 7) Disseminate the final guidelines with the software engineering research community through conferences, workshops, and academic journals. Engage with the community to promote adopting and using the guidelines in practice. 8) Regularly review and update the guidelines in light of new developments in ChatGPT technology, ethical concerns, and feedback from the research community. Ensure they remain relevant and effective in addressing the ethical challenges of using ChatGPT in software engineering research.


==> relationship.tex <==
\section{Relationship of motivators and demotivators with ethical aspects (principles)}
\label{sec:relationship}

Preliminary, we develop a taxonomy by considering the identified motivators, demotivators, and their possible impact on ChatGPT ethics aspects. Motivators are factors that encourage or inspire researchers to consider ChatGPT as a tool for people to take certain actions. At the same time, demotivators discourage or hinder people from taking certain actions. In this context, motivators and demotivators may refer to factors that influence the use of ChatGPT in software engineering research. The taxonomy considers the possible impact of these motivators and demotivators on the ethical aspects of using ChatGPT in software engineering research. Ethics aspects (principles) refer to the moral standards that guide behavior and decision-making in software engineering research.  The proposed taxonomy (Figure \ref{Fig.Mapping of motivators and demotivators against research ethics}) provides a roadmap for academic researchers to evaluate both the motivators (positive factors) and demotivators (negative factors) related to the ethical aspects of using ChatGPT in software engineering research. By considering these factors, researchers can gain a comprehensive understanding of the ethical considerations associated with using ChatGPT in software engineering research. This taxonomy can serve as a valuable tool for researchers to ensure that they use ChatGPT ethically and responsibly. It can also contribute to developing ethical guidelines and best practices for using ChatGPT in software engineering research.

\begin{figure*}[htbp]
\centerline{\includegraphics[width=\linewidth]{Images/ChatGPT-Ethics-Taxonomy-Taxonomy.drawio.pdf}}
\caption{Mapping of motivators and demotivators against research ethics}
\label{Fig.Mapping of motivators and demotivators against research ethics}
\end{figure*}

